The Marseille Schmidt survey for active star-forming galaxies. I. Data on 92 emission line objects in two fields

We present data from a moderately deep spectroscopic Schmidt survey (Blim=17.5) of ``active galaxies'' selected by the presence of emission lines in their spectra and/or their UV excess. The redshift, magnitudes, color and diameter reduction methods have been discussed in a previous paper. Here we explain the emission line equivalent width determination method. 92 emission line objects have been found in two adjacent fields (approximately 50deg^2) in the direction of the south extension of the Virgo cluster. We give a catalog containing positions, photographic R and B magnitudes, U-R colors, effective diameters, redshifts, equivalent widths and intensity ratios of the [OIII]4959,5007, Hbeta and [OII] 3727 emission lines. On these fields, we evaluate the completeness limit of the survey at a pseudo B magnitude value of 15.7.

==> art2TB_3_mssfits.tex <==
%%\input aa.cmm
\hsize=210truemm
\vsize=290truemm
\hoffset=-25truemm
\voffset=0truemm
\baselineskip=12.045truept
\parindent=2.5em
%%\nopagenumbers
\def\ub{\underbar}
\def\right#1{\quad#1\hfill}
\def\left#1{\hfill#1\quad}
\def\cen#1{\quad#1\quad}
\def\noa#1{\noalign{\hskip 10pt}#1}
\def\comment#1{\noalign{{\hskip 20truemm }\vbox{\hsize=160truemm \parindent=0.0em{#1}}}}
\def\commentitem#1{\noalign{{\hskip 25truemm }{\hsize=160truemm \parindent=0.0em{\bf #1}}}}
\def\sp5{\noindent\hangindent=2.5em}
\def\etal{{\it et al.}}
\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sevenrm=cmr7
\font\sixrm=cmr6
\font\fiverm=cmr5
\font \bf = cmr10
%%\font \bf = cmbx10 at 09truept
%%at 08truept
\font \it = cmti10 at 09truept
%%at 08truept
%%\ninerm
%%\eightrm
%%\sevenrm
%%\sixrm
\fiverm
%%{\bf n} & {\bf name } & {\bf ident } 
%%& {\bf ha } & {\bf ma } & {\bf sa } & {\bf dd} & {\bf md} & {\bf sd }
%%&{\bf Hvel } & {\bf $\delta v$ } 
%%& {\bf  morph } 
%%& {\bf mR } & {\bf R } & {\bf U-R } & {\bf mB} 
%%& {\bf $w_{OIII}$ } & {\bf $w_{H\beta}$ } & {\bf $w_{OII}$ } 
%%& {\bf Deff} \cr


$$
\vbox {\halign
{\hfill# & \quad#\hfill &\quad#\hfill 
&\quad#\hfill&\hfill#\hfill & \hfill#\quad 
&\hfill#\hfill &\hfill#\hfill &\hfill#\quad 
&\hfill#\ & \hfill#\quad 
& #\hfill 
&\hfill# & \hfill# &\hfill# & \hfill#
& \hfill# & \hfill# & \hfill#\quad 
& \hfill# & \hfill#
& \hfill#\cr 
\noalign{\hrule}
\noalign{\vskip 10pt}
\hfill{\bf (1)}\hfill & \hfill{\bf (2)}\hfill &\hfill {\bf (3) } \hfill
& \multispan{3} \hfill {\bf (4)} \hfill & \multispan{3} \hfill {\bf (5)} \hfill 
& \hfill{\bf (6) } \hfill& \hfill{\bf (7) \hfill} 
& \hfill{\bf  (8) } \hfill
& \hfill{\bf (9) }\hfill &\hfill {\bf (10) }\hfill &\hfill {\bf (11) }\hfill & \hfill{\bf (12)}\hfill 
& \hfill{\bf (13) } \hfill& \hfill{\bf (14) } \hfill& \hfill{\bf (15)}\hfill
& \hfill{\bf (16)}\hfill&\hfill {\bf (17)}\hfill & \hfill{\bf (18) }\hfill\cr
\hfill{\bf n}\hfill & \hfill{\bf name }\hfill &\hfill {\bf ident } \hfill
& \multispan{6} \hfill {\bf $\alpha$ \hfill (1950) \hfill $\delta$} \hfill 
& \hfill{\bf Hvel } \hfill& \hfill{\bf $\delta v$ \hfill} 
& \hfill{\bf  morph } \hfill
& \hfill{\bf mR }\hfill &\hfill {\bf R }\hfill &\hfill {\bf U-R }\hfill & \hfill{\bf mB}\hfill 
& \hfill{\bf $w_{\eightrm OIII}$ } \hfill& \hfill{\bf $w_{\eightrm H\beta}$ } \hfill& \hfill{\bf $w_{\eightrm OII}$}\hfill
& \hfill{\bf {\eightrm $[OIII]\over H\beta$}}\hfill&\hfill {\bf {\eightrm $[OII]\over [OIII]$}}\hfill & \hfill{\bf Deff }\hfill\cr
\noalign{\vskip 10pt}
\noalign{\hrule}
\noalign{\vskip 2pt}
\noalign{\hrule}
\noalign{\vskip 10pt}
    &            &            &    &    &      &     &    &    &      &     &         &       &       &     &        &     &     &     &     &     &      \cr
  1 & 13016-2237 &            & 13 &  1 & 34.0 & -22 & 36 & 55 & 2886 & 48 & BC        & 17.0 & -15.9 & 1.7 & 18.0   & 85 &     & 551&     & 0.60& 0.95 \cr      
  2 & 13020-1851 &            & 13 &  2 &  2.5 & -18 & 50 & 56 & 13386& 173& Sp        & 15.4 & -20.9 & 1.9 & 17.0   & 36 &  9 & 19 & 4.10& 0.21& 8.30 \cr      
  3 & 13021-2343 &            & 13 &  2 &  8.7 & -23 & 42 & 58 & 6656 & 70 & BC        & 17.0 & -17.7 & 3.4 & 18.2   &     &     &     &     &     & 2.07 \cr      
  4 & 13024-1956 &            & 13 &  2 & 25.5 & -19 & 56 & 10 & 11079& 311& ?         & 17.7 & -18.2 & 2.2 & 18.7   &     &     &     &     &     & 4.21 \cr      
  5 & 13024-1957a&            & 13 &  2 & 22.0 & -19 & 56 & 30 & 7411 & 246& Irr/SP    & 16.2 & -18.8 & 2.1 & 17.1   &     &     &     &     &     & 4.83 \cr      
  6 & 13024-1957b&            & 13 &  2 & 22.5 & -19 & 56 & 32 & 7194 & 247& companion & 18.1 & -16.8 & 2.1 & 19.0   &     &     &     &     &     & 2.17 \cr      
  7 & 13026-2229 &            & 13 &  2 & 36.6 & -22 & 28 & 55 & 15098& 451& Sp?       & 16.0 & -20.5 & 2.4 & 17.4   &     &     &     &     &     & 7.81 \cr      
  8 & 13027-2314 &            & 13 &  2 & 43.7 & -23 & 14 &  2 & 3213 & 100& BC        & 16.0 & -17.2 & 1.8 & 17.5   & 322&     & 46 & 7.58&     & 1.31 \cr      
  9 & 13034-2221 & CTS 1029   & 13 &  3 & 23.5 & -22 & 21 & 18 & 10515& 100& ?         & 17.2 & -18.5 & 1.9 & 18.4   & 64 & 98 & 216& 0.86& 0.74& 3.15 \cr      
 10 & 13036-2119 &            & 13 &  3 & 37.5 & -21 & 18 & 30 & 12666& 122& Irr?      & 15.9 & -20.2 & 1.9 & 17.0   & 29 & 15 & 45 & 1.87& 0.92& 8.51 \cr      
 11 & 13036-2243 &NPM-22.0244 & 13 &  3 & 37.8 & -22 & 42 & 44 & 2906 & 42 & BC        & 15.4 & -17.6 & 2.4 & 16.5 $^*$ & 68 & 13 & 46 & 5.11& 0.31& 1.50 \cr   
 12 & 13040-2211 &ESO 575-055 & 13 &  3 & 58.4 & -22 & 11 & 19 & 2543 & 191& Sp        & 14.6 & -18.1 & 2.4 & 16.0 $^*$ &     &     &     &     &     & 1.53 \cr   
 13 & 13042-2234 & ESO 508-04 & 13 &  4 & 10.5 & -22 & 34 & 23 & 2725 & 176& Sp/IP     &      &       &     & 15.1   &     &     &     &     &     &      \cr      
 14 & 13044-2325 & NGC4968    & 13 &  4 & 24.1 & -23 & 24 & 34 & 3042 & 217& Sp/AGN    & 13.0 & -20.0 & 3.4 & 13.7 $^*$ & 46 &     &     &     &     & 3.29 \cr   
 15 & 13044-2022 &            & 13 &  4 & 25.1 & -20 & 21 & 46 & 13850& 488& Sp/AGN?   &      &       &     & 18.7   &     &     &     &     &     &      \cr      
 16 & 13046-2600 &            & 13 &  4 & 36.9 & -26 &  0 &  9 & 14464& 49 & Sp/AGN?   & 17.1 & -19.4 & 1.8 & 17.8   &     &     &     &     &     & 6.80 \cr      
 17 & 13050-2631 &            & 13 &  4 & 57.3 & -26 & 31 &  0 & 13202& 36 & Sp        & 16.3 & -19.9 & 1.8 & 17.4   &     &     &     &     &     & 5.16 \cr      
 18 & 13051-2235 & ESO508-11  & 13 &  5 &  3.1 & -22 & 35 & 25 & 2659 & 34 & Sp        &      &       &     & 13.8 $^*$ & 160& 39 & 282& 4.50& 0.19&      \cr   
 19 & 13056-1841 &            & 13 &  5 & 38.9 & -18 & 40 & 41 & 14189& 70 & BC        & 16.3 & -20.1 & 1.9 & 17.5   & 127&     & 50 &     & 0.27& 4.75 \cr      
 20 & 13058-2033 &            & 13 &  5 & 48.7 & -20 & 33 & 27 & 580  & 112& Irr       & 15.6 & -13.9 & 2.1 & 16.8   &     &     &     &     &     & 0.28 \cr      
 21 & 13060-2407 &I13059-2407 & 13 &  5 & 59.6 & -24 &  6 & 59 & 4019 & 100& SY2/Sp    & 14.6 & -19.0 & 2.9 & 16.2 $^*$ &     &     &     &     &     & 2.56 \cr   
 22 & 13064-2021 &            & 13 &  6 & 26.0 & -20 & 20 & 30 & 15311& 103&  ?        & 17.9 & -18.7 & 2.0 & 19.1   & 84 & 37 & 175 & 2.43& 0.43& 3.96 \cr      
 23 & 13066-2407 & ESO 508-15 & 13 &  6 & 36.1 & -24 &  6 & 53 & 3001 & 100& Irr/clump &      &       &     & 14.5   & 45 &     & 104&     & 0.36&      \cr      
 24 & 13072-2358 & ESO 508-19 & 13 &  7 &  9.1 & -23 & 58 & 24 & 3147 & 46 & Irr/B     &      &       &     & 14.3 $^*$ & 46 & 16 & 29 & 2.91& 0.30&      \cr   
 25 & 13073-2627 & ESO 508-21 & 13 &  7 & 17.0 & -26 & 26 & 35 & 2100 & 68 & Sp/B nucl &      &       &     & 16.3 $^*$ &     &     &     &     &     &      \cr   
 26 & 13078-2119 &            & 13 &  7 & 47.3 & -21 & 19 & 14 & 7240 & 139& ?         &      &       &     & 15.7   &     &     &     &     &     &      \cr        
 27 & 13079-2129 & ESO 576-03 & 13 &  7 & 53.9 & -21 & 28 & 57 & 3281 & 100& Sp/B HIIr &      &       &     & 14.0 $^*$ & 48 & 14 & 79 & 3.57& 0.69&      \cr     
 28 & 13081-2336 & ESO 508-24 & 13 &  8 &  3.5 & -23 & 35 & 59 & 2725 & 72 & Sp/B nucl &      &       &     & 13.7 $^*$ &     &     &     &     &     &      \cr    
 29 & 13082-2041 & ESO 576-40 & 13 &  8 &  9.5 & -20 & 41 & 24 & 11426& 65 & I.P       &      &       &     & 16.3 $^*$ &     &     &     &     &     &      \cr     
 30 & 13084-2745 & ESO 443-80 & 13 &  8 & 24.5 & -27 & 44 & 33 & 2214 & 25 & Sp/B      &      &       &     & 13.8 $^*$ & 145& 30 & 25 & 5.51& 0.22&      \cr     
 31 & 13084-1938 &            & 13 &  8 & 25.4 & -19 & 37 & 40 & 13127& 180& Sp ?      & 16.1 & -20.1 & 2.1 & 17.3   &     &     &     &     &     & 8.03 \cr        
 32 & 13085-1902 &            & 13 &  8 & 29.1 & -19 &  1 & 45 & 15855& 77 & ?         & 18.2 & -18.5 & 1.4 & 29.3   & 331& 77 & 40 & 3.54& 0.33& 4.97 \cr        
 33 & 13088-2604 &            & 13 &  8 & 46.4 & -26 &  3 & 41 & 9060 & 36 & BC        & 16.1 & -19.4 & 2.2 & 17.6   &     &     &     &     &     & 3.57 \cr      
 34 & 13090-2016 &            & 13 &  9 &  1.5 & -20 & 16 & 20 & 2353 & 75 & Irr/B     & 14.7 & -17.8 & 2.1 & 15.6   &     &     &     &     &     & 1.70 \cr      
 35 & 13095-1919 & NPM-19.0446& 13 &  9 & 27.1 & -19 & 19 & 19 & 7082 & 615& Irr/B     & 15.8 & -19.0 & 2.1 & 17.0   &     &     &     &     &     & 3.77 \cr     
 36 & 13095-2631 &            & 13 &  9 & 31.1 & -26 & 30 & 34 & 9183 & 23 & ?         & 17.1 & -18.3 & 1.7 & 18.7   & 265& 49 & 126& 5.76& 0.23& 3.47 \cr        
 37 & 13098-2530 &            & 13 &  9 & 47.0 & -25 & 30 &  0 & 15550& 100& ?         & 17.7 & -18.9 & 2.0 & 16.2   &     &     &     &     &     & 3.68 \cr      
 38 & 13098-2501 & CTS 0021   & 13 &  9 & 45.2 & -25 &  1 &  6 & 19002& 373& SY1       & 16.0 & -21.0 & 2.1 & 17.5 $^*$ &     & 30 &     &     &     & 6.85 \cr     
 39 & 13107-1918 &            & 13 & 10 & 39.1 & -19 & 17 & 59 & 10825& 113& Sp/B      & 15.8 & -20.0 & 1.8 & 16.7   &     &     &     &     &     & 6.34 \cr      
 40 & 13114-2124 & ESO 576-15 & 13 & 11 & 26.5 & -21 & 23 & 48 & 3568 & 41 & Sp/B/LSB? &      &       &     & 17.2 $^*$ & 176& 107& 11 & 2.35& 0.34&      \cr     
 41 & 13118-2506 &            & 13 & 11 & 49.4 & -25 &  6 & 22 & 7816 & 24 & ?         & 17.1 & -17.9 & 1.7 & 18.4   & 204& 45 & 83 & 4.81& 0.18& 3.11 \cr      
 42 & 13120-2038 &            & 13 & 11 & 58.7 & -20 & 37 & 38 & 12404& 343& ?         &      &       &     & 17.1   &     &     &     &     &     &      \cr      
 43 & 13122-2149 &            & 13 & 12 & 13.4 & -21 & 48 & 59 & 5624 & 100& Sp        &      &       &     & 17.1   & 197& 41 &     & 4.88&     &      \cr      
 44 & 13124-2432 &            & 13 & 12 & 21.0 & -24 & 32 & 11 & 12132& 65 & Irr/B     & 16.4 & -19.7 & 1.6 & 17.0   &     &     &     &     &     &      \cr      
 45 & 13124-1913 &            & 13 & 12 & 22.3 & -19 & 13 & 28 & 7933 & 70 & BC        & 16.0 & -19.1 & 2.0 & 17.4   &     &     &     &     &     & 2.79 \cr      
 46 & 13126-2535 &            & 13 & 12 & 33.0 & -25 & 34 & 34 & 13171& 63 & Sp/Irr/B  & 17.3 & -19.0 & 1.4 & 17.7   &     &     &     &     &     &      \cr      
    &            &            &    &    &      &     &    &    &      &    &           &      &       &     &        &     &     &     &     &     &      \cr
\noalign{\vskip 10pt}
\noalign{\hrule}
}}$$
\vfill
\eject



$$\vbox {\halign 
{\hfill# & \quad#\hfill &\quad#\hfill 
&\quad#\hfill&\hfill#\hfill & \hfill#\quad 
&\hfill#\hfill &\hfill#\hfill &\hfill#\quad 
&\hfill#\ & \hfill#\quad 
& #\hfill 
&\hfill# & \hfill# &\hfill# & \hfill#
& \hfill# & \hfill# & \hfill#\quad 
& \hfill# & \hfill#
& \hfill#\cr 
\noalign{\hrule}
\noalign{\vskip 10pt}
\hfill{\bf (1)}\hfill & \hfill{\bf (2)}\hfill &\hfill {\bf (3) } \hfill
& \multispan{3} \hfill {\bf (4)} \hfill & \multispan{3} \hfill {\bf (5)} \hfill 
& \hfill{\bf (6) } \hfill& \hfill{\bf (7) \hfill} 
& \hfill{\bf  (8) } \hfill
& \hfill{\bf (9) }\hfill &\hfill {\bf (10) }\hfill &\hfill {\bf (11) }\hfill & \hfill{\bf (12)}\hfill 
& \hfill{\bf (13) } \hfill& \hfill{\bf (14) } \hfill& \hfill{\bf (15)}\hfill
& \hfill{\bf (16)}\hfill&\hfill {\bf (17)}\hfill & \hfill{\bf (18) }\hfill\cr

\hfill{\bf n}\hfill & \hfill{\bf name }\hfill &\hfill {\bf ident } \hfill
& \multispan{6} \hfill {\bf $\alpha$ \hfill (1950) \hfill $\delta$} \hfill 
& \hfill{\bf Hvel } \hfill& \hfill{\bf $\delta v$ \hfill} 
& \hfill{\bf  morph } \hfill
& \hfill{\bf mR }\hfill &\hfill {\bf R }\hfill &\hfill {\bf U-R }\hfill & \hfill{\bf mB}\hfill 
& \hfill{\bf $w_{\eightrm OIII}$ } \hfill& \hfill{\bf $w_{\eightrm H\beta}$ } \hfill& \hfill{\bf $w_{\eightrm OII}$}\hfill
& \hfill{\bf {\eightrm $[OIII]\over H\beta$}}\hfill&\hfill {\bf {\eightrm $[OII]\over [OIII]$}}\hfill & \hfill{\bf Deff }\hfill\cr
\noalign{\vskip 10pt}
\noalign{\hrule}
\noalign{\vskip 2pt}
\noalign{\hrule}
\noalign{\vskip 10pt}
    &            &            &    &    &      &     &    &    &      &    &           &      &       &     &        &     &     &     &     &     &      \cr
 47 & 13125-1944 &            & 13 & 12 & 30.8 & -19 & 43 & 31 & 6418 & 123& BC        & 17.4 & -17.3 & 2.2 & 18.8   & 140& 32 &     & 4.64&     & 2.70 \cr      
 48 & 13125-2006a&            & 13 & 12 & 32.4 & -20 &  5 & 50 & 7642 & 234& Sp/B/LSB  &      &       &     & 17.4   &     &     &     &     &     &      \cr      
    & 13125-2006b&            & 13 & 12 & 32.8 & -20 &  5 & 52 & 8194 & 94 & ?         &      &       &     &        &     &     &     &     &     &      \cr      
 49 & 13128-2343 & NGC 5042   & 13 & 12 & 47.9 & -23 & 43 & 12 & 1352 & 57 & Sp HIIr   &      &       &     & 12.2 $^*$ & 482& 146& 238& 5.28& 0.18&      \cr   
 50 & 13136-2618 & ESO 508-33 & 13 & 13 & 38.8 & -26 & 17 & 50 & 3259 & 41 & Sp/AGN    & 13.4 & -19.8 & 2.5 & 15.0 $^*$ & 6 & 7 & 25 & 0.86 & 1.97 & 2.56 \cr    
 51 & 13137-2420 &            & 13 & 13 & 44.5 & -24 & 20 & 23 & 1581 & 177& Sp   nucl &      &       &     & 17.0   &     &     &     &     &     &      \cr      
 52 & 13140-2737 & ESO 444-02 & 13 & 13 & 59.8 & -27 & 37 & 21 & 1693 & 23 & Sp  HIIr  &      &       &     & 15.0 $^*$ & 158& 33 & 52 & 5.02& 0.25&      \cr    
 53 & 13141-2449 &            & 13 & 14 &  8.8 & -24 & 49 & 21 & 13705& 53 & I.P ?     & 16.0 & -20.3 & 1.7 & 17.0   & 77 & 29 & 102& 2.82& 5.87& 0.81 \cr      
 54 & 13156-2113 &            & 13 & 15 & 38.0 & -21 & 12 & 31 & 16117& 70 & Sp?       & 15.6 & -21.1 & 3.9 & 17.3   & 56 &     &     &     &     & 9.24 \cr      
 55 & 13160-1849 & ESO 576-27 & 13 & 15 & 59.8 & -18 & 49 &  1 & 3082 & 70 & Sp        & 13.9 & -19.2 & 2.3 & 14.7 $^*$  & 19 & 15 & 31 & 1.30& 0.79& 3.02 \cr     
 56 & 13162-2304 &I13161-2304 & 13 & 16 &  9.3 & -23 &  4 & 23 & 15497& 49 & SP/B/LSB  & 15.2 & -20.4 & 2.9 & 16.5   & 27 & 16 & 266& 1.72& 0.74&11.03 \cr        
 57 & 13162-2046 &            & 13 & 16 & 13.1 & -20 & 45 & 30 & 8655 & 70 & ?         &      &       &     & 18.4   &     &     &     &     &     &      \cr      
 58 & 13162-2047 & NGC 5068   & 13 & 16 & 12.1 & -20 & 46 & 36 & 504  & 70 & HIIr      &      &       &     &         & 951&     & 479& 2.36& 0.74&      \cr      
    & 13162-2047 &            & 13 & 16 & 12.1 & -20 & 46 & 36 & 800  & 70 & SP nucl   &      &       &     & 10.7 $^*$   &     &     &     & 3.22& 0.23&      \cr      
 59 & 13163-2513 &            & 13 & 16 & 19.5 & -25 & 12 & 36 & 12068& 45 & ?         & 18.3 & -17.8 & 1.3 & 18.9   &     &     &     &     &     & 2.36 \cr      
 60 & 13172-2335 &            & 13 & 17 & 10.1 & -23 & 34 & 45 & 2177 & 68 & Sp        & 15.4 & -16.9 & 2.1 & 16.3   & 83 & 17 & 112& 5.15& 0.42&      \cr      
 61 & 13173-1944 &            & 13 & 17 & 18.7 & -19 & 43 & 36 & 6262 & 50 & Irr/Sp    & 15.2 & -19.4 & 2.0 & 16.3   & 224& 54 & 41 & 3.90& 0.31& 5.57 \cr      
 62 & 13176-2317 & I13176-2316& 13 & 17 & 38.6 & -23 & 16 & 45 & 13784& 100& Sp  nucl  & 15.0 & -21.3 & 2.9 & 16.8   & 26 & 68 & 14 & 3.66& 0.22& 8.91 \cr      
 63 & 13177-2549 & ESO 508-51 & 13 & 17 & 44.9 & -25 & 49 & 24 & 1981 & 43 & Sp  nucl  &      &       &     & 14.3 $^*$ & 29 & 10 & 25 & 2.97& 0.43&      \cr   
 64 & 13181-2313 &IF13181-2312& 13 & 18 &  5.9 & -23 & 13 &  9 & 1860 & 42 & I.P       & 15.7 & -16.3 & 1.9 & 17.0   & 33 & 5  & 77 & 7.13& 0.66& 1.43 \cr      
 65 & 13181-2034 &            & 13 & 18 &  6.0 & -20 & 34 & 20 & 3138 & 324& ?         & 18.2 & -14.9 & 1.7 & 18.8 &     &     &     &     &     & 0.97 \cr        
 66 & 13183-2027 &            & 13 & 18 & 15.8 & -20 & 26 & 39 & 14106& 243& Irr ,I.P  & 15.9 & -20.5 & 2.3 & 17.2 &     &     &     &     &     & 8.35 \cr        
 67 & 13194-2214 &            & 13 & 19 & 24.0 & -22 & 14 & 21 & 9074 & 54 & BC        & 16.6 & -18.8 & 2.3 & 18.3 & 59 & 10 & 61 & 6.08& 0.44&      \cr        
 68 & 13191-2213 &            & 13 & 19 &  6.9 & -22 & 12 & 51 & 7164 & 148& BC        & 16.4 & -18.5 & 2.3 & 17.6   & 30 & 9  & 34 & 2.16& 1.01&      \cr      
 69 & 13192-2514 & ESO 508-59 & 13 & 19 & 10.1 & -25 & 13 & 56 & 2204 & 27 & SP/ HIIr  &      &       &     & 15.1 $^*$ & 129& 16 & 50 & 8.38& 0.16&      \cr   
 70 & 13195-2211 &            & 13 & 19 & 27.5 & -22 & 11 &  0 & 9538 & 147& Sp ?      & 16.3 & -19.2 & 2.6 & 18.3   &     &     &     &     &     & 3.65 \cr      
 71 & 13196-1905 &            & 13 & 19 & 34.1 & -19 &  4 & 55 & 5060 & 70 & LSB/B ?   & 16.6 & -17.6 & 1.9 & 17.8   &     &     &     &     &     & 2.80 \cr      
 72 & 13198-2020 &            & 13 & 19 & 45.1 & -20 & 20 &  5 & 6189 & 70 & Sp/AGN ?  & 17.5 & -17.1 & 2.0 & 18.3   & 230&     &     &     &     & 1.57 \cr  
 73 & 13206-2536 &IF13205-2536& 13 & 20 & 33.0 & -25 & 35 & 59 & 10192& 61 & Sp/AGN    & 15.5 & -20.2 & 2.5 & 17.3   &     &     &     &     &     & 4.96 \cr      
 74 & 13210-2724 & Abell 1736 & 13 & 20 & 59.4 & -27 & 23 & 58 & 2388 & 54 & SY2       & 15.5 & -17.0 & 1.9 & 17.0 $^*$& 25 & 5 & 10& 4.44 & 0.32 & 0.82 \cr      
 75 & 13211-1926 & NPM-19.0448& 13 & 21 &  7.7 & -19 & 26 & 10 & 5305 & 206& Sp/AGN    & 16.0 & -18.3 & 2.0 & 17.0   &     &     &     &     &     & 2.54 \cr     
 76 & 13214-1935 &            & 13 & 21 & 24.0 & -19 & 34 & 48 & 7788 & 116& Irr/B?    & 16.8 & -18.3 & 1.9 & 17.8   &     &     &     &     &     & 3.55 \cr      
 77 & 13214-2337 & ESO 508-67 & 13 & 21 & 26.2 & -23 & 37 &  0 & 7362 & 38 & Sp/I.P    & 13.9 & -21.0 & 2.4 & 15.3 $^*$ & 13 & 6 & 2.34 & 0.84 & 31&      \cr   
 78 & 13217-2435 &            & 13 & 21 & 40.6 & -24 & 34 & 58 & 9404 & 136& ?         & 18.0 & -17.5 & 1.9 & 18.9   &     &     &     &     &     & 3.25 \cr      
 79 & 13217-2023 &            & 13 & 21 & 43.6 & -20 & 23 & 24 & 8120 & 163& ?         & 16.9 & -18.3 & 1.8 & 18.1   & 71 & 11 & 44 & 6.54& 0.32&      \cr      
 80 & 13218-2023 & NPM-20.0399& 13 & 21 & 48.0 & -20 & 23 & 14 & 8044 & 90 & Sp/AGN?   & 15.5 & -19.6 & 2.0 & 16.7   &     &     &     &     &     & 3.69 \cr     
 81 & 13220-1926 & ESO 576-50 & 13 & 21 & 59.5 & -19 & 26 &  8 & 2232 & 100& Sp/B+comp?&      &       &     & 13.2 $^*$ &3439& 75 & 56 & 6.51& 0.21&      \cr     
 82 & 13223-2410 &            & 13 & 22 & 15.7 & -24 &  9 & 45 & 1594 & 31 & Irr/Sp    & 16.2 & -15.5 & 2.2 & 17.0   & 38 & 16 & 50 & 2.22& 0.46& 1.61 \cr      
 83 & 13225-2614 & I13225-2614& 13 & 22 & 30.6 & -26 & 14 & 14 & 18440& 51 & Sp/Irr    & 15.6 & -21.4 & 2.0 & 16.6 $^*$ &     &     &     &     &     & 8.83 \cr   
 84 & 13228-2540 &            & 13 & 22 & 48.7 & -25 & 40 &  0 & 4523 & 34 & Sp/Irr    &      &       &     & 17.5   & 191& 40 & 97 & 4.80& 0.21&      \cr      
 85 & 13228-1954 &            & 13 & 22 & 45.9 & -19 & 54 &  8 & 8721 & 141& Irr/sp    & 15.2 & -20.1 & 2.1 & 16.7   & 35 & 4  & 27 & 7.46& 0.58& 3.80 \cr      
 86 & 13228-1955 &IF13227-1954& 13 & 22 & 47.6 & -19 & 55 &  4 & 8345 & 90 & Irr,I.P   & 16.0 & -19.3 & 1.9 & 17.6   &     &     &     & 5.56& 0.24&      \cr      
 87 & 13228-1955 &IF13227-1954& 13 & 22 & 47.6 & -19 & 54 & 50 & 7862 & 101& Irr,I.P   & 17.3 & -17.8 & 1.5 & 16.7   &     &     &     & 5.83& 0.36&      \cr      
 88 & 13228-2547 &            & 13 & 22 & 47.6 & -25 & 47 & 13 & 4458 & 70 & BC        & 17.9 &       &     & 17.9   & 52 & 5  & 54 & 9.55& 0.50&      \cr      
 89 & 13229-2118 &            & 13 & 22 & 53.0 & -21 & 18 & 20 & 8405 & 70 & Irr/B     & 16.0 & -19.3 & 1.8 & 16.8   & 150&     &     &     &     & 4.76 \cr      
 90 & 13230-1958 &            & 13 & 23 &  0.7 & -19 & 58 & 29 & 2299 & 119& Irr       & 15.9 & -16.5 & 2.2 & 17.0   &     &     &     &     &     &      \cr     
 91 & 13232-2323 & CTS 1031   & 13 & 23 & 14.4 & -23 & 22 & 33 & 13421& 85 & Sp        &      &       &     & 18.9   & 328& 78 & 532& 4.84& 0.28&      \cr      
 92 & 13243-2742 & ESO 444-39 & 13 & 24 & 19.9 & -27 & 41 & 49 & 2023 & 37 & Sp/B      & 13.6 & -18.6 & 2.2 & 14.9   & 190& 41 & 42 & 4.83& 0.15& 1.97 \cr     
    &            &            &    &    &      &     &    &    &      &    &           &      &       &     &        &     &     &     &     &     &      \cr
\noalign{\vskip 10pt}
\noalign{\hrule}
}}$$
\vfill
\eject
\end
% 93 &            &            &    &    &      &     &    &    & 10747& 232&           &       &        &      &         & 387& 36 & 235&     &     &      \cr
% 94 &            &            &    &    &      &     &    &    & 15663& 247&           &       &        &      &         & 620& 179&     &     &     &      \cr

